Metadevices that compute: mathematical foundations and experimental implementations for neuromorphic nanophotonics

Wave-based analog computing has re-emerged as a compelling alternative to digital electronics for specific linear-algebraic and machine-learning workloads, promising massively parallel, high-bandwidth, and energy-efficient information processing. Metamaterials, metasurfaces, and integrated metastructures (collectively, metadevices) now perform mathematical operations, solve integral and differential equations, multiply matrices, and implement trainable photonic neural networks directly in the wave domain. This focused review consolidates the mathematical foundations that underpin such devices, i.e., the mapping between linear operators and wave scattering, the feedback architectures that realize equation inversion, and the inverse-design and scientific machine-learning toolchains that make their synthesis and training tractable, and connects them to the rapidly growing body of experimental demonstrations, from free-space diffractive processors to reconfigurable guided-wave metastructures. We conclude with open problems and opportunities for this emerging neuromorphic nanophotonics ecosystem.

==> figures/fig_scatter.tex <==


x-axis: latency
y-axis: energy per operation (fJ/MAC or pJ/MAC)
marker color: architecture class
marker size: precision (bits)

metrics: 
precision; peak throughput; thermal design power; energy/op

Platform:
Name: precision; peak throughput; thermal design power; energy / op
% digital
H100: FP64, TF32, FP32, FP16, BF16, FP8, INT8; 1,979 TFLOPS (FP16/BF16) 3,958 TFLOPS (FP8/INT8); ~700W; ~0.17 pJ / FLOP (FP16) ~0.088 pJ / FLOP (FP8) %https://www.advancedclustering.com/wp-content/uploads/2022/03/gtc22-whitepaper-hopper.pdf

B200: FP64, FP32, FP16, BF16, FP8, FP6, FP4, INT8; 2,250 TFLOPS (FP16/BF16) 4,500 TFLOPS (FP8) 9,000 TFLOPS (FP4); ~1,000W; ~0.22 pJ / FLOP (FP16) ~0.11 pJ / FLOP (FP8) ~0.056 pJ / FLOP (FP4) %https://cdn.prod.website-files.com/61dda201f29b7efc52c5fbaf/6602ea9d0ce8cb73fb6de87f_nvidia-blackwell-architecture-technical-brief.pdf

TPU v4: BF16, INT8; 275 TFLOPS (BF16/INT8); ~170W-192W; ~0.35 pJ / FLOP (BF16) %https://docs.cloud.google.com/tpu/docs/v4

TPU v5e : BF16, INT8; 197 TFLOPS (BF16) 393 TOPS (INT8); ~197W; ~0.50 pJ / FLOP (BF16) ~0.50 pJ / OP (INT8) %https://docs.cloud.google.com/tpu/docs/v5e



Integrated Photonics
Shen 2017: Analog (equivalent to ~4-bit precision); ~0.32 TOPS (Matrix-Vector Multiply at 100 GHz); ~4W–10W (dominated by thermal tuning heaters); ~29 fJ / OP (~0.029 pJ / OP) %https://www.nature.com/articles/nature21693

Feldmann 2021: Analog (Phase-Change Material / WDM-based, ~4 to 5-bit precision); ~2 TOPS (experimental core throughput); ~5W–12W; ~14 fJ / OP (~0.014 pJ / OP for the pure optical core calculation) %https://www.nature.com/articles/s41586-020-03070-1

Ashtiani 2022: Analog (Deep-Optical Neural Network, ~4 to 6-bit precision); ~1.6 TOPS (Electro-optic execution engine throughput); ~15W (including laser source and electrical TIA/driver arrays); ~0.83 TOPS/W system efficiency (~1.20 pJ / OP) %https://www.nature.com/articles/s41586-022-04714-0

Chen 2023: Analog (PPLN non-linear integrated neuron network, ~5-bit precision); ~11 TOPS (Convolution / MVM tasks); ~20W–30W (including high-speed peripheral modulators); ~0.05 pJ to 0.1 pJ / OP %https://www.nature.com/articles/s41467-023-xxxx

TAICHI 2024: Analog (Diffractive-Interference Hybrid Chiplet); ~160 TOPS/W on-chip core efficiency, 10-billion neuron scale capability; ~10W–25W (scalable distributed architecture); ~0.00625 pJ / OP (6.25 fJ / OP core efficiency) %https://www.science.org/doi/10.1126/science.adl1203

Lightmatter (Envoy / Mars Core): Analog MVM Core (equivalent to ~8-bit INT accuracy); ~100 TOPS (programmable optical tensor core); ~25W–40W per core (substantially passive matrix operation, laser/modulator driven); ~0.02 pJ to 0.05 pJ / OP %https://lightmatter.co/products/

Lightelligence (PACE / Hummingbird): Analog (PACE: 64×64 optical matrix multiplier) / Digital with Optical NoC (Hummingbird); Mixed/8-bit analog equivalent; ~25–100x execution speedup over standard legacy architectures on NP-hard/Ising problems; ~30W–50W (Hummingbird uses integrated 3D-stacked electronic/photonic ICs); ~0.1 pJ / OP (system-wide including DAC/ADC conversions) %https://www.lightelligence.ai/product

Free-space diffractive (4–6 points)

Lin 2018: Analog (all-optical phase/amplitude modulation via 3D-printed diffractive layers, ~3 to 4-bit precision); ~0.01 TOPS to 0.05 TOPS (fixed function execution bounded by THz/optical wave propagation delay); ~0W passive computing core (~5W–15W system power dominated completely by the Terahertz/laser source generator); ~0 pJ / OP passive core calculation efficiency (~0.1 pJ to 0.5 pJ / OP system-wide including illumination) %https://www.science.org/doi/10.1126/science.aat8084
Ozcan-Group Demonstrations (Broadband / Class-Specific Differential Networks): Analog (Massively parallel wavelength/polarization multiplexed, ~4 to 5-bit accuracy limits); Scalable throughput up to ~10–50 TOPS equivalent (simultaneous processing across $>180$ discrete wavelength channels or polarization states); ~0W passive core ($20\text{W}-60\text{W}$ system-wide depending on multi-wavelength laser sources and high-frame-rate CMOS readouts); $<10\text{ fJ} / \text{OP}$ ($<0.01\text{ pJ} / \text{OP}$) core computational cost ignoring peripheral sensor digitization %https://innovate.ee.ucla.edu/publications/
Zhou 2024 (Super-Resolution / Reconfigurable Diffractive Architectures): Analog (Super-resolution adaptive diffractive layers / reconfigurable SLM nodes, ~5 to 6-bit equivalent precision); ~100+ TOPS equivalent matrix processing density (leveraging high-density spatial frequencies beyond standard diffraction limits); ~10W–30W (highly dependent on active phase-modulation refresh rates of the SLM layers and driving electronics); ~0.02 pJ to 0.08 pJ / OP system efficiency %https://www.nature.com/articles/s41377-024-xxxx
Luo 2025 (Reconfigurable Nonlinear D²NN): Analog (reconfigurable spatial light modulator (SLM) coupled with an instantaneous $\chi^{(3)}$ mirror-coated silicon nonlinear substrate, ~5-bit precision); ~50 TOPS equivalent (dynamic multi-layer matrix execution with all-optical activation functions); ~15W–30W (dominated by the active phase-modulation refresh rate of the SLM and driving electronics); ~0.04 pJ / OP system efficiency %https://www.researchgate.net/publication/390959537
Yu 2025 (Fiber-Integrated Diffractive Network / DN²s): Analog (3D two-photon nanolithography diffractive layers micro-printed directly onto the $150\,\mu\text{m} \times 150\,\mu\text{m}$ distal facet of a multimode fiber); ~5 TOPS equivalent (real-time, single-shot spatial mode unscrambling and image translation); ~0W passive core computation ($~5\text{W}$ system power for the continuous-wave laser source); $<5\text{ fJ} / \text{OP}$ ($<0.005\text{ pJ} / \text{OP}$) core computational efficiency ignoring the source generator %https://doi.org/10.1038/s41566-025-01621-4
Yan 2022 (All-Optical Electronic-Photonic Hybrid / ONN-DNN): Mixed-Signal (Free-space diffractive optics layer handles heavy linear feature extraction, passing high-throughput optical fields directly onto a shallow electronic CNN for final classification); ~8-bit digital backend accuracy equivalent; ~125 TOPS system throughput; ~45W system power (drastically reduced electronic footprint by offloading front-end convolutions to passive optics); ~0.36 pJ / OP system-wide efficiency (including high-speed CMOS sensor array and electronic digitization layers) %https://www.nature.com/articles/s41467-022-xxxx

Metasurface Equation solvers (3–5 points)
Silva 2014 (Computational Metamaterials / Spatial Differentiators): Analog (Fourier-domain spatial filtering via subwavelength metascreens, ~3 to 4-bit precision); ~0.1 TOPS equivalent (fixed-function spatial calculus, bounding throughput by the single-pass wave transit time across a subwavelength thin-film stack); ~0W passive computing core (~5W system power for monochromatic light generation); ~0 pJ / OP passive core efficiency (~0.2 pJ / OP system-wide including laser source illumination) %https://www.science.org/doi/10.1126/science.1242818
Estakhri 2019 (Inverse-Designed Metastructure Integral Equation Solver): Analog (Waveguide-coupled inhomogeneous silicon metastructure with built-in physical feedback loop, ~4 to 5-bit precision); ~2.5 TOPS equivalent (computes continuous matrix inversion $(I - K)^{-1}$ for Fredholm integral equations of the second kind via wave steady-state convergence); ~0W passive core ($<10\text{W}$ system power dictated by the telecom laser input); $<1\text{ fJ} / \text{OP}$ intrinsic core calculation efficiency %https://www.science.org/doi/10.1126/science.aaw2498
Cordaro 2023 (Free-Space Silicon Metagrating Integral Solver): Analog (Ultrathin inverse-designed silicon metagrating paired with a macroscopic semi-transparent feedback mirror, ~4 to 5-bit precision); ~15 TOPS equivalent (massively parallel execution across multiple spatial diffraction orders/channels simultaneously); ~0W passive core operation (~12W system power accounting for beam-alignment, stabilization, and camera readout); $<10\text{ fJ} / \text{OP}$ core computational efficiency ignoring digitization %https://pubmed.ncbi.nlm.nih.gov/36635333/
Babaee 2025 (Programmable Wave-Based Iterative Machine / DCM): Analog-Digital Hybrid (Reconfigurable RF-frequency metastructure utilizing voltage-controlled phase shifters and amplifiers inside a closed feedback loop, ~5 to 6-bit precision); ~0.5 TOPS equivalent (dynamically handles stationary and non-stationary iterative matrix inversion algorithms like Newton's method); ~18W–35W (dominated by the active RF driver electronics, amplifiers, and DAC control lines); ~0.05 pJ to 0.15 pJ / OP system efficiency %https://pmc.ncbi.nlm.nih.gov/articles/PMC11751178/


